From Sensor to Processing Networks: Optimal Estimation with Computation and Communication Latency

This paper investigates the use of a networked system ($e.g.$, swarm of robots, smart grid, sensor network) to monitor a time-varying phenomenon of interest in the presence of communication and computation latency. Recent advances in edge computing have enabled processing to be spread across the network, hence we investigate the fundamental computation-communication trade-off, arising when a sensor has to decide whether to transmit raw data (incurring communication delay) or preprocess them (incurring computational delay) in order to compute an accurate estimate of the state of the phenomenon of interest. We propose two key contributions. First, we formalize the notion of $processing$ $network$. Contrarily to $sensor$ $and$ $communication$ $networks$, where the designer is concerned with the design of a suitable communication policy, in a processing network one can also control when and where the computation occurs in the network. The second contribution is to provide analytical results on the optimal preprocessing delay ($i.e.$, the optimal time spent on computations at each sensor) for the case with a single sensor and multiple homogeneous sensors. Numerical results substantiate our claims that accounting for computation latencies (both at sensor and estimator side) and communication delays can largely impact the estimation accuracy.

==> Sections/brownian-motion.tex <==
%!TEX root = ../processing_networks_estimation.tex

\myParagraph{Example: Brownian systems}
% \begin{exmp}[Brownian systems]
An interesting case arises when the system~\eqref{scalar-system} describes a Brownian motion
\begin{equation}
\begin{cases}
dx_t = dw_t\\
z_t(\tau) = x_t + v_t(\tau)
\end{cases} \label{scalar-system-a-eq-0}
\end{equation}
since the optimal delay has a simple expression.

\begin{cor}[Brownian motion]
		Given system (\ref{scalar-system-a-eq-0}) and hypotheses as per Theorem~\ref{thm-scalar}, the steady-state error variance $\psteadytau(\tau)$ has the following expression:
		\begin{equation*}
		\psteadytau(\tau) = \underbrace{\sqrt{\dfrac{b\sigma^2_w}{\tau}}}_{f(\tau)} + \underbrace{\sigma^2_w\tau}_{q(\tau)}
		\end{equation*}
		admitting the unique global minimum
		\begin{equation}
		\tau^\text{B}_{opt} = \sqrt[3]{\dfrac{b}{4\sigma^2_w}}
		\label{tmin-a-eq-0}
		\end{equation}
\end{cor}
% \end{exmp}

Notice that the cubic root in (\ref{tmin-a-eq-0}) strongly reduces $ \tau^\text{B}_{opt}$ sensitivity to system parameters, which may be useful with model uncertainty.
Also, the contribution $ f(\tau) $ decreases with the square root of $\tau$, while $ q(\tau) $ grows linearly.
%model uncertainties are important.

==> Sections/fig-paramDependence.tex <==
%!TEX root = ../processing_networks_estimation.tex

\begin{figure}[b]
\centering
\begin{minipage}{.5\textwidth}
	\centering
	\includegraphics[width=.7\textwidth]{Images/tau_of_s.eps}\vspace{-3mm}
	\caption{$\tau_{opt}(s)$, with $a=1$ and upper bound $\tau_{u}(|a|,s)$.}
	\label{fig:tau_of_s}
\end{minipage}
%		\begin{minipage}{.45\textwidth}
%			\centering
%			\includegraphics[width=.85\textwidth]{Images/tau_of_a2.eps}\vspace{-3mm}
%			\caption{$\tau_{opt}(a^2)$, with $s=1$.}
%			\label{fig:tau_of_a2}
%		\end{minipage}
\end{figure}

==> Sections/homogeneous-network.tex <==
%!TEX root = ../processing_networks_estimation.tex

\subsection{Sensor selection in homogeneous networks}\label{sec:discussion-hom-net}



==> Sections/proof-thm-param-dep.tex <==
	\section{Proof of Proposition \ref{prop-params}} \label{app:proof-prop-params}
	
	For this proof we are going to exploit the implicit function theorem, whose statement is recalled for convenience.
	\begin{thm}[Dini's theorem]
		Let F be a continuously differentiable function on some open $D \subset \mathbb{R}^2$. Assume that there exists a point $(\bar{x},\bar{y}) \in D$ such that:
		\begin{itemize}
			\item $F(\bar{x},\bar{y})=0$;
			\item $\dfrac{\partial F}{\partial y}(\bar{x},\bar{y})\neq 0$.
		\end{itemize}
		Then, there exist two positive constant a, b and a function $f : I_{\bar{x}}:=(\bar{x}-a,\bar{x}+a) \mapsto J_{\bar{y}}:=(\bar{y}-b,\bar{y}+b)$ such that
		\[F(x,y)=0 \iff y = f(x) \quad \forall x \in I_{\bar{x}}, \ \forall y \in J_{\bar{y}}\]
		Moreover, $f \in \mathcal{C}^1(I_{\bar{x}})$ and
		\[ f'(x) = -\frac{F_x(x,f(x))}{F_y(x,f(x))} \quad \forall x \in I_{\bar{x}}\]
%		where $F_x(x,f(x)) = \frac{\partial F}{\partial x}(x,f(x))$.
		\label{thm-Dini}
	\end{thm}
	We can see the left-hand term in eq. (\ref{3rd-degree-eq-scalar-general}) as a one-parameter function of two positive-valued variables, namely
	\[ F: \mathbb{R}_+ \times \mathbb{R}_+ \rightarrow \mathbb{R}, \ (\pi,\tau) \mapsto F(\pi,\tau) = s\tau^3 + a^2\tau^2-\frac{1}{4}\]
	with $\pi=\{s,a^2\}$. First of all, let us check if Dini's theorem hypotheses are satisfied: given a solution $(\bar{\pi}, \bar{\tau}_{opt})$ of eq. (\ref{3rd-degree-eq-scalar-general}) it holds
	\begin{itemize}
		\item $F(\bar{\pi}, \bar{\tau}_{opt}) = 0$, by construction;
		\item $F_{\tau}(\bar{\pi}, \bar{\tau}_{opt}) = 3s\bar{\tau}_{opt}^2 +2a^2\bar{\tau}_{opt} > 0$, since all variables are positive.
	\end{itemize}
	Then Thm. \ref{thm-Dini} applies and there exists a function $\tau(\pi)$ such that $F(\pi,\tau_{opt}) = 0 \iff \tau_{opt} = \tau(\pi)$, with $\pi$ in some open neighbourhood of $\bar{\pi}$. In fact, since we did not pose constraints on $(\bar{\pi}, \bar{\tau}_{opt})$, we can state that such a function is defined for all $ \pi\in\mathbb{R}_+ $. The two cases for $\pi$ are studied independently.
	\begin{description}
		\item[$\boldsymbol{\pi = s}$] 
		By Thm. \ref{thm-Dini}, the first derivative of $\tau(\pi) = \tau(s)$ is
		\begin{equation}
		\tau'(s) = -\dfrac{F_{s}(s,\tau(s))}{F_{\tau}(s,\tau(s))} = -\dfrac{{\tau(s)}^2}{3{s}{\tau(s)} +2a^2} \label{tau-of-s-derivative}
		\end{equation}
		We conclude that $\tau'(s) < 0 \ \forall s \in \mathbb{R}_+$, namely, $\tau_{opt}$ is strictly decreasing with $s$.
		
		\item[$\boldsymbol{\pi = a^2}$] The first derivative of $\tau(\pi) = \tau(a^2)$ is
		\begin{align}
		\tau'(a^2) &= -\dfrac{F_{a^2}(a^2,\tau(a^2))}{F_{\tau}(a^2,\tau(a^2))} = -\dfrac{\tau(a^2)}{3s{\tau(a^2)} +2a^2} \label{tau-of-a-derivative}
		\end{align}
		We conclude that $\tau'(a^2) < 0 \ \forall a \in \mathbb{R}$, namely, $\tau_{opt}$ is strictly decreasing with $a^2$, regardless of sign$(a)$.
	\end{description}

==> Sections/proof-thm-prep-comm-del.tex <==
\section{Proof of Theorem \ref{thm-scalar-total}} \label{app:proof-thm-scalar-total}
	
By applying open-loop prediction to $ p_{\infty}(\tau) $ to cover the total delay $ \tau+\tau_c(\tau) $, the steady-state prediction error variance can be written as in eq. (\ref{p-prep-comm-del}). Critical point analysis leads to the following identity:
\begin{equation*}
	\dfrac{\sigma^2_w}{b}\tau^5+a^2\tau^4-\frac{2c\sigma^2_w}{b}\tau^3-\left(2a^2c+\frac{1}{4}\right)\tau^2+\dfrac{c^2\sigma^2_w}{b}\tau+a^2c^2 = 0
	\label{eq-5-deg}
\end{equation*}
Being all coefficients positive, Cartesio's rule ensures that it admits two positive solutions, yielding a unique point of global minimum, and possibly a maximum (or saddle) for asymptotically stable systems.
%	\footnote{Such possibility comes from squaring the terms of an equation with a square root inside it, thus not always admitting both the final solutions.}
Moreover, by observing that $\lim_{\tau \rightarrow +\infty}p'_{\infty+\tau_{tot}|\infty}(\tau) = 0^+$ (the variance asymptotically grows), we conclude that the point of minimum is always greater than the other critical point. The maximum brings a local minimum at $ \tau = 0 $.

==> Sections/proof-thm-prep-del.tex <==
%!TEX root = ../processing_networks_estimation.tex

	\section{Proof of Theorem \ref{thm-scalar}}\label{app:proof-thm-scalar}
	
	By considering the variance model~\eqref{sigmav-of-tau}, the steady-state Kalman error variance for system~\eqref{scalar-system} can be written as
	\begin{equation}
	p_\infty(\tau) = \frac{{b}}{\tau}\left(a+\sqrt{a^2+\frac{\sigma^2_w}{{b}}\tau}\right) \label{p-infty}
	\end{equation}	
	Model-based open-loop prediction has error dynamics
	\begin{equation}
	d\Tilde{x}_{s|t}(\tau) = a\Tilde{x}_{s|t}(\tau)dt + dw_s, \qquad s\ge t
	\label{open-loop-error-dynamics-scalar}
	\end{equation}
	Then, prediction error at time $t+\tau$ is given by solving (\ref{open-loop-error-dynamics-scalar}) as a Cauchy problem with initial condition $\Tilde{x}_t$:
	\begin{equation*}
	\Tilde{x}_{t+\tau|t}(\tau) = \mbox{e}^{a\tau}\Tilde{x}_t(\tau)+\Bar{w}_t
	\end{equation*}
	where $\Bar{w}_t$ is the stochastic integral of $ w_s $ in the interval $[t,\: t+\tau]$. The steady-state prediction error variance is then 
	\begin{align*}
	\begin{split}
	p_{\infty+\tau|\infty}(\tau) &\overset{(i)}{=} \mbox{var}(\mbox{e}^{a\tau}\Tilde{x}_t) + \mbox{var}(\Bar{w}_t) =\\
	& = \frac{{b}\mbox{e}^{2a\tau}}{\tau}\left(a+\sqrt{a^2+\frac{\sigma^2_w}{{b}}\tau}\right)+\frac{\sigma^2_w}{2a}\left(\mbox{e}^{2a\tau}-1\right)
	\end{split}
	\end{align*}
	where $(i)$ is motivated by $\Tilde{x}_t$ and $\Bar{w}_t$ being uncorrelated. Indeed, $\tilde{x}_t \in \mbox{span}\{x_{t_0}, w_s, v_s : t_0 \le s\le t\}$, while $\Bar{w}_t \in \mbox{span}\{w_s, \: t \le s \le t+\tau\}$, with $w_t$ white noise and $w_t \perp x_{t_0}, v_s \ \forall t\ge t_0,\forall s$ by hypothesis. The only sample providing nonzero correlation is $w_t$, but having zero Lebesgue measure its contribution to $\Bar{w}_t$ is null.\\
	We proceed now in studying critical points of $ p_{\infty+\tau|\infty}(\tau) $, since being limits~\eqref{error-variance-limits-scalar} equal at both domain extrema and being $  p_{\infty+\tau|\infty}(\tau)  \in\mathcal{C}^0(\bar{\mathbb{R}}_+)$ at least one must exist. By setting $ p_{\infty+\tau|\infty}'(\tau)=0 $ and rejecting $\tau=0$, we get
	\begin{equation}
	\frac{\sigma^2_w}{b}\tau^3 + a^2\tau^2-\frac{1}{4} = 0 
	\label{3rd-degree-eq-scalar-general-1}
	\end{equation}
	
	This equation always admits a real positive solution, in virtue of Bolzano's theorem by considering $F(\tau):=\nicefrac{\sigma^2_w}{b}\tau^3 + a^2\tau^2-\nicefrac{1}{4}$ and $I:=\left[0,\nicefrac{1}{2|a|}\right]$. Quasi-convexity of $ p_{\infty+\tau|\infty}(\tau) $ can be checked by looking at its sublevel sets, which are (convex) intervals: this guarantees that the critical point is indeed the unique point of global minimum.
